Time Series Data Augmentation for Neural Networks by Time Warping with a Discriminative Teacher

Neural networks have become a powerful tool in pattern recognition and part of their success is due to generalization from using large datasets. However, unlike other domains, time series classification datasets are often small. In order to address this problem, we propose a novel time series data augmentation called guided warping. While many data augmentation methods are based on random transformations, guided warping exploits the element alignment properties of Dynamic Time Warping (DTW) and shapeDTW, a high-level DTW method based on shape descriptors, to deterministically warp sample patterns. In this way, the time series are mixed by warping the features of a sample pattern to match the time steps of a reference pattern. Furthermore, we introduce a discriminative teacher in order to serve as a directed reference for the guided warping. We evaluate the method on all 85 datasets in the 2015 UCR Time Series Archive with a deep convolutional neural network (CNN) and a recurrent neural network (RNN). The code with an easy to use implementation can be found at https://github.com/uchidalab/time_series_augmentation .

==> icprfull.tex <==
@article{sakoe1978dynamic,
  title={Dynamic programming algorithm optimization for spoken word recognition},
  author={Sakoe, Hiroaki and Chiba, Seibi},
  journal={IEEE Trans. Acoustics, Speech, and Sig. Process.},
  volume={26},
  number={1},
  pages={43--49},
  year={1978},
  publisher={IEEE}
}

@inproceedings{ratanamahatana2004everything,
  title={Everything you know about dynamic time warping is wrong},
  author={Ratanamahatana, Chotirat A and Keogh, Eamonn},
  year={2004},
  pages={53--63},
  booktitle = {Workshop Mining Temporal and Sequential Data},
}

@article{itakura1975minimum,
  title={Minimum prediction residual principle applied to speech recognition},
  author={Itakura, Fumitada},
  journal={IEEE Trans. Acoustics, Speech, and Sig. Process.},
  volume={23},
  number={1},
  pages={67--72},
  year={1975},
  publisher={IEEE}
}

@article{Shorten_2019,
	doi = {10.1186/s40537-019-0197-0},
	year = 2019,
	publisher = {Springer},
	volume = {6},
	number = {1},
	author = {Connor Shorten and Taghi M. Khoshgoftaar},
	title = {A survey on Image Data Augmentation for Deep Learning},
	journal = {J. Big Data}
}

@misc{UCRArchive,
title={The UCR Time Series Classification Archive},
author={ Chen, Yanping and Keogh, Eamonn and Hu, Bing and Begum, Nurjahan and Bagnall, Anthony and Mueen, Abdullah and Batista, Gustavo},
year={2015},
note = {\url{www.cs.ucr.edu/~eamonn/time_series_data/}}
}

 @misc{UCRArchive2018,
    title = {The UCR Time Series Classification Archive},
    author = {Dau, Hoang Anh and Keogh, Eamonn and Kamgar, Kaveh and Yeh, Chin-Chia Michael and Zhu, Yan 
              and Gharghabi, Shaghayegh and Ratanamahatana, Chotirat Ann and Yanping and Hu, Bing 
              and Begum, Nurjahan and Bagnall, Anthony and Mueen, Abdullah and Batista, Gustavo, and Hexagon-ML},
    year = {2018},
    note = {\url{https://www.cs.ucr.edu/~eamonn/time_series_data_2018/}}
}

@inproceedings{brain1999on,
  title={On the effect of data set size on bias and variance in classification learning},
  author={Brain, Damien and Geoffrey Webb},
  year={1999},
  pages={117--128},
  booktitle = {Australian Knowl. Acq. Workshop},
}

@inproceedings{Banko_2001,
	doi = {10.3115/1073012.1073017},
	year = 2001,
	author = {Michele Banko and Eric Brill},
	title = {Scaling to very very large corpora for natural language disambiguation},
	booktitle = {Annual Meeting Assoc. Comput. Ling.}
}

@article{Torralba_2008,
	doi = {10.1109/tpami.2008.128},
	year = 2008,
	publisher = {IEEE},
	volume = {30},
	number = {11},
	pages = {1958--1970},
	author = {A. Torralba and R. Fergus and W.T. Freeman},
	title = {80 Million Tiny Images: A Large Data Set for Nonparametric Object and Scene Recognition},
	journal = {{IEEE} Trans. Pattern Anal. and Mach. Intell.}
}

@inproceedings{NIPS2019_9035,
title = {Fixing the train-test resolution discrepancy},
author = {Touvron, Hugo and Vedaldi, Andrea and Douze, Matthijs and Jegou, Herve},
booktitle = {Adv. in Neural Inform. Process. Sys.},
pages = {8252--8262},
year = {2019},
}

@inproceedings{Edunov_2018,
	doi = {10.18653/v1/d18-1045},
	year = 2018,
	author = {Sergey Edunov and Myle Ott and Michael Auli and David Grangier},
	pages = {489--500},
	title = {Understanding Back-Translation at Scale},
	booktitle = {Conf. Empir. Meth. in Nat. Lang. Process.}
}

@article{verma2019learning,
    title={Learning Universal Graph Neural Network Embeddings With Aid Of Transfer Learning},
    author={Saurabh Verma and Zhi-Li Zhang},
  journal={arXiv preprint arXiv:1909.10086},
  year={2019}
}

@article{Schmidhuber_2015,
	doi = {10.1016/j.neunet.2014.09.003},
	year = 2015,
	publisher = {Elsevier},
	volume = {61},
	pages = {85--117},
	author = {Jürgen Schmidhuber},
	title = {Deep learning in neural networks: An overview},
	journal = {Neural Networks}
}

@article{ILSVRC15,
Author = {Olga Russakovsky and Jia Deng and Hao Su and Jonathan Krause and Sanjeev Satheesh and Sean Ma and Zhiheng Huang and Andrej Karpathy and Aditya Khosla and Michael Bernstein and Alexander C. Berg and Li Fei-Fei},
Title = {ImageNet Large Scale Visual Recognition Challenge},
Year = {2015},
journal   = {Int. J. Comput. Vis.},
doi = {10.1007/s11263-015-0816-y},
volume={115},
number={3},
pages={211-252}
}

@article{Lecun_1998,
	doi = {10.1109/5.726791},
	year = 1998,
	publisher = {IEEE},
	volume = {86},
	number = {11},
	pages = {2278--2324},
	author = {Y. Lecun and L. Bottou and Y. Bengio and P. Haffner},
	title = {Gradient-based learning applied to document recognition},
	journal = {Proc. {IEEE}}
}

@article{krizhevsky2009learning,
  title={Learning Multiple Layers of Features from Tiny Images},
  author={Krizhevsky, Alex},
  year={2009}
}

@InProceedings{IsmailFawaz2018,
  Title                    = {Data augmentation using synthetic data for time series classification with deep residual networks},
  Author                   = {Ismail Fawaz, Hassan and Forestier, Germain and Weber, Jonathan and Idoumghar, Lhassane and Muller, Pierre-Alain},
  Booktitle                = {Int. Workshop Adv. Anal. and Temporal Data},
  Year                     = {2018}
}


@inproceedings{le2016data,
  title={Data augmentation for time series classification using convolutional neural networks},
  author={{Le Guennec}, Arthur and Malinowski, Simon and Tavenard, Romain},
  booktitle={Int. Workshop Adv. Anal. and Temporal Data},
  year={2016}
}

@inproceedings{Um_2017,
	doi = {10.1145/3136755.3136817},
	year = 2017,
	author = {Terry T. Um and Franz M. J. Pfister and Daniel Pichler and Satoshi Endo and Muriel Lang and Sandra Hirche and Urban Fietzek and Dana Kuli{\'{c}}},
	title = {Data augmentation of wearable sensor data for parkinson's disease monitoring using convolutional neural networks},
	pages = {216--220},
	booktitle = {ACM Int. Conf. Multimodal Interaction}
}

@inproceedings{Rashid_2019,
	doi = {10.22260/isarc2019/0087},
	year = 2019,
	author = {Khandakar M. Rashid and Joseph Louis},
	title = {Time-Warping: A Time Series Data Augmentation of {IMU} Data for Construction Equipment Activity Identification},
	booktitle = {Int. Symp. Auto. and Robot. in Construction}
}

@article{wen2020time,
  title={Time Series Data Augmentation for Deep Learning: A Survey},
  author={Wen, Qingsong and Sun, Liang and Song, Xiaomin and Gao, Jingkun and Wang, Xue and Xu, Huan},
  journal={arXiv preprint arXiv:2002.12478},
  year={2020}
}

@inproceedings{Forestier_2017,
	doi = {10.1109/icdm.2017.106},
	year = 2017,
	author = {Germain Forestier and Francois Petitjean and Hoang Anh Dau and Geoffrey I. Webb and Eamonn Keogh},
	title = {Generating Synthetic Time Series to Augment Sparse Datasets},
	booktitle = {IEEE Int. Conf. Data Mining}
}

@article{Kamycki_2019,
	doi = {10.3390/s20010098},
	year = 2019,
	publisher = {{MDPI} {AG}},
	volume = {20},
	number = {1},
	pages = {98},
	author = {Krzysztof Kamycki and Tomasz Kapuscinski and Mariusz Oszust},
	title = {Data Augmentation with Suboptimal Warping for Time-Series Classification},
	journal = {Sensors}
}

@inproceedings{yu2017seqgan,
  title={Seqgan: Sequence generative adversarial nets with policy gradient},
  author={Yu, Lantao and Zhang, Weinan and Wang, Jun and Yu, Yong},
  booktitle={AAAI Conf. Artificial Intell.},
  year={2017}
}

@inproceedings{nikolaidis2019augmenting,
  title={Augmenting Physiological Time Series Data: A Case Study for Sleep Apnea Detection},
  author={Nikolaidis, Konstantinos and Kristiansen, Stein and Goebel, Vera and Plagemann, Thomas and Liest{\o}l, Knut and Kankanhalli, Mohan},
  booktitle={European Conf. Mach. Learning and Principles of Knowl. Discovery in Databases},
  year={2019}
}

@article{Harada_2019,
	doi = {10.1109/access.2019.2934928},
	year = 2019,
	publisher = {IEEE},
	volume = {7},
	pages = {144292--144302},
	author = {Shota Harada and Hideaki Hayashi and Seiichi Uchida},
	title = {Biosignal Generation and Latent Variable Analysis With Recurrent Generative Adversarial Networks},
	journal = {{IEEE} Access}
}

@inproceedings{NIPS2019_8789,
title = {Time-series Generative Adversarial Networks},
author = {Yoon, Jinsung and Jarrett, Daniel and van der Schaar, Mihaela},
booktitle = {Adv. Neural Inform. Process. Sys.},
pages = {5508--5518},
year = {2019},
}


@article{Wendling_2000,
	doi = {10.1007/s004220000160},
	year = 2000,
	publisher = {Springer },
	volume = {83},
	number = {4},
	pages = {367--378},
	author = {F. Wendling and J. J. Bellanger and F. Bartolomei and P. Chauvel},
	title = {Relevance of nonlinear lumped-parameter models in the analysis of depth-{EEG} epileptic signals},
	journal = {Bio. Cybernetics}
}

@inproceedings{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and Pouget-Abadie, Jean and Mirza, Mehdi and Xu, Bing and Warde-Farley, David and Ozair, Sherjil and Courville, Aaron and Bengio, Yoshua},
booktitle = {Adv. in Neural Inform. Process. Sys.},
  pages={2672--2680},
  year={2014}
}

@article{simonyan2014very,
  title={Very deep convolutional networks for large-scale image recognition},
  author={Simonyan, Karen and Zisserman, Andrew},
  journal={arXiv preprint arXiv:1409.1556},
  year={2014}
}

@inproceedings{He_2016,
	doi = {10.1109/cvpr.2016.90},
	year = 2016,
	author = {Kaiming He and Xiangyu Zhang and Shaoqing Ren and Jian Sun},
	title = {Deep Residual Learning for Image Recognition},
	booktitle = {{IEEE/CVF} Conf. Comput. Vis. and Pattern Recogn.}
}

@inproceedings{Cui_2014,
	doi = {10.1109/icassp.2014.6854671},
	year = 2014,
	author = {Xiaodong Cui and Vaibhava Goel and Brian Kingsbury},
	title = {Data Augmentation for deep neural network acoustic modeling},
	booktitle = {{IEEE} Int. Conf. Acoustics, Speech and Sig. Process.}
}

@article{Tran_2020,
	doi = {10.1109/access.2020.2966142},
	year = 2020,
	publisher = {IEEE},
	volume = {8},
	pages = {12364--12378},
	author = {Lam Tran and Deokjai Choi},
	title = {Data Augmentation for Inertial Sensor-Based Gait Deep Neural Network},
	journal = {{IEEE} Access}
}

@article{Delgado_Escano_2019,
	doi = {10.1109/access.2018.2886899},
	year = 2019,
	publisher = {IEEE},
	volume = {7},
	pages = {1897--1908},
	author = {Ruben Delgado-Escano and Francisco M. Castro and Julian Ramos Cozar and Manuel J. Marin-Jimenez and Nicolas Guil},
	title = {An End-to-End Multi-Task and Fusion {CNN} for Inertial-Based Gait Recognition},
	journal = {{IEEE} Access}
}

@inproceedings{jaitly2013vocal,
  title={Vocal tract length perturbation (VTLP) improves speech recognition},
  author={Jaitly, Navdeep and Hinton, Geoffrey E},
  booktitle={ICML Workshop Deep Learning for Audio, Speech, and Lang. Processing},
  year={2013}
}

@inproceedings{Takahashi_2016,
	doi = {10.21437/interspeech.2016-805},
	year = 2016,
	author = {Naoya Takahashi and Michael Gygli and Beat Pfister and Luc Van Gool},
	title = {Deep Convolutional Neural Networks and Data Augmentation for Acoustic Event Recognition},
	booktitle = {Interspeech}
}

@article{Petitjean_2011,
	doi = {10.1016/j.patcog.2010.09.013},
	year = 2011,
	publisher = {Elsevier},
	volume = {44},
	number = {3},
	pages = {678--693},
	author = {Fran{\c{c}}ois Petitjean and Alain Ketterlin and Pierre Gan{\c{c}}arski},
	title = {A global averaging method for dynamic time warping, with applications to clustering},
	journal = {Pattern Recogn.}
}

@inproceedings{Kim_2019,
	doi = {10.21437/interspeech.2019-3227},
	year = 2019,
	author = {Chanwoo Kim and Minkyu Shin and Abhinav Garg and Dhananjaya Gowda},
	title = {Improved Vocal Tract Length Perturbation for a State-of-the-Art End-to-End Speech Recognition System},
	booktitle = {Interspeech}
}

@article{Schuster_1997,
	doi = {10.1109/78.650093},
	year = 1997,
	volume = {45},
	number = {11},
	pages = {2673--2681},
	author = {M. Schuster and K.K. Paliwal},
	title = {Bidirectional recurrent neural networks},
	journal = {{IEEE} Trans. Sig. Process.}
}

@article{reimers2017optimal,
  title={Optimal hyperparameters for deep lstm-networks for sequence labeling tasks},
  author={Reimers, Nils and Gurevych, Iryna},
  journal={arXiv preprint arXiv:1707.06799},
  year={2017}
}

@article{Hochreiter_1997,
	doi = {10.1162/neco.1997.9.8.1735},
	year = 1997,
	publisher = {{MIT} Press},
	volume = {9},
	number = {8},
	pages = {1735--1780},
	author = {Sepp Hochreiter and Jürgen Schmidhuber},
	title = {Long Short-Term Memory},
	journal = {Neural Computation}
}

@article{cho2014learning,
  title={Learning phrase representations using RNN encoder-decoder for statistical machine translation},
  author={Cho, Kyunghyun and Van Merri{\"e}nboer, Bart and Gulcehre, Caglar and Bahdanau, Dzmitry and Bougares, Fethi and Schwenk, Holger and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1406.1078},
  year={2014}
}

@article{Zhao_2018,
	doi = {10.1016/j.patcog.2017.09.020},
	year = 2018,
	publisher = {Elsevier},
	volume = {74},
	pages = {171--184},
	author = {Jiaping Zhao and Laurent Itti},
	title = {{shapeDTW}: Shape Dynamic Time Warping},
	journal = {Pattern Recogn.}
}

@article{Kenji_Iwana_2020,
	doi = {10.1016/j.patcog.2019.107024},
	year = 2020,
	publisher = {Elsevier},
	volume = {97},
	pages = {107024},
	author = {Brian Kenji Iwana and Seiichi Uchida},
	title = {Time series classification using local distance-based features in multi-modal fusion networks},
	journal = {Pattern Recogn.}
}

@article{dozat2016incorporating,
  title={Incorporating nesterov momentum into adam},
  author={Dozat, Timothy},
  year={2016}
}

@inproceedings{Iwana_2019,
	doi = {10.1109/icassp.2019.8682908},
	year = 2019,
	author = {Brian Kenji Iwana and Seiichi Uchida},
	title = {Dynamic Weight Alignment for Temporal Convolutional Neural Networks},
	booktitle = {{IEEE} Int. Conf. Acoustics, Speech and Sig. Process.},
	pages={3827--3831}
}

@inproceedings{Wu_2019,
	doi = {10.1109/icassp.2019.8683036},
	year = 2019,
	author = {Xiaomeng Wu and Akisato Kimura and Seiichi Uchida and Kunio Kashino},
	title = {Prewarping Siamese Network: Learning Local Representations for Online Signature Verification},
	booktitle = {{IEEE} Int. Conf. Acoustics, Speech and Sig. Process.},
	pages={2467--2471}
}

@article{iwana2017efficient,
  title={Efficient temporal pattern recognition by means of dissimilarity space embedding with discriminative prototypes},
  author={Iwana, Brian Kenji and Frinken, Volkmar and Riesen, Kaspar and Uchida, Seiichi},
  journal={Pattern Recogn.},
  volume={64},
  pages={268--276},
  year={2017},
  doi={10.1016/j.patcog.2016.11.013},
}

@article{Bagnall_2016,
	doi = {10.1007/s10618-016-0483-9},
	year = 2016,
	publisher = {Springer},
	volume = {31},
	number = {3},
	pages = {606--660},
	author = {Anthony Bagnall and Jason Lines and Aaron Bostrom and James Large and Eamonn Keogh},
	title = {The great time series classification bake off: a review and experimental evaluation of recent algorithmic advances},
	journal = {Data Mining and Knowl. Discovery}
}

@inproceedings{Bagnall_2016_COTE,
	doi = {10.1109/icde.2016.7498418},
	year = 2016,
	author = {Anthony Bagnall and Jason Lines and Jon Hills and Aaron Bostrom},
	title = {Time-series classification with {COTE}: The collective of transformation-based ensembles},
	booktitle = {{IEEE} Int. Conf. Data Eng.}
}

@article{Hills_2013,
	doi = {10.1007/s10618-013-0322-1},
	year = 2013,
	publisher = {Springer},
	volume = {28},
	number = {4},
	pages = {851--881},
	author = {Jon Hills and Jason Lines and Edgaras Baranauskas and James Mapp and Anthony Bagnall},
	title = {Classification of time series by shapelet transformation},
	journal = {Data Mining and Knowl. Discovery}
}

@article{Pearson_1901,
	doi = {10.1080/14786440109462720},
	year = 1901,
	publisher = {Informa},
	volume = {2},
	number = {11},
	pages = {559--572},
	author = {Karl Pearson},
	title = {On lines and planes of closest fit to systems of points in space},
	journal = {The London, Edinburgh, and Dublin Philo. Mag. and J. Sci.}
}
